Searching for the 511 keV annihilation line from galactic compact objects with the IBIS gamma ray telescope

The first detection of a gamma ray line with an energy of about 500 keV from the center our Galaxy dates back to the early seventies. Thanks to the astrophysical application of high spectral resolution detectors, it was soon clear that this radiation was due to the 511 keV photons generated by electron-positron annihilation. Even though the physical process are known, the astrophysical origin of this radiation is still a mystery. The spectrometer SPI aboard the INTEGRAL gamma-ray satellite has been used to produce the first all-sky map in light of the 511 keV annihilation, but no direct evidence for 511 keV galactic compact objects has been found [...] We present the first deep IBIS 511 keV all-sky map, obtained by applying standard analysis to about 5 years of data. Possible 511 keV signals are also searched over hour-day-month timescales. The IBIS sensitivity at 511 keV depends on the detector quantum efficiency at this energy and on the background. Both these quantities were estimated in this work. We find no evidence of Galactic 511 keV point sources. With an exposure of 10 Ms in the center of the Galaxy, we estimate a $1.6 \times 10^{-4}\,ph\,cm^{-2}\,s^{-1}$ flux 2 sigma upper limit. A similar limit is given in a wide area in the Galactic center region with similar exposures. The IBIS 511 keV flux upper limits for microquasars and supernova remnants detected in the hard X domain ($E > 20\, keV$) are also reported. Our results are consistent with a diffuse $e^{+}e^{-}$ annihilation scenario. If positrons are generated in compact objects, we expect that a significant fraction of them propagate in the interstellar medium before there are annihilated away from their birth places.

==> mc-simulation.tex <==
   Another way to evaluate the sensitivity is through a Monte Carlo simulation of an on-axis point source with an energy of 511~keV. The 511~keV sky image, obtained after {\em shadowgram} decoding, is shown in Fig. \ref{fig:sim511-withbkg}. To obtain this result we have generated a parallel photons beam impinging perpendicularly onto the IBIS mask surface. Then the event file produced by the Monte Carlo was processed in order to obtain the ISGRI detector {\em shadowgram} and then the reconstructed image. We use now this kind of simulation to estimate the IBIS/ISGRI sensitivity at 511~keV. Before the decoding algorithm, we add an uniform background to the first {\em shadowgram}, which include only the source photons. 

   In our simulation the background count rate is taken from the data accumulated during revolution 50 (Fig. \ref{fig:isgri_spec}). We simulate a 511~keV flux of $10^{-2}\, ph\, cm^{-2}\, s^{-1}$ with an exposure of $100\, ks$. Since the sensitivity depends on the square root of the exposure (Equation \ref{eq:sens}), this observation corresponds to a flux of $10^{-3}\, ph\, cm^{-2}\, s^{-1}$ with an exposure of $10\, Ms$,  that is the maximum exposure of our data set (Fig. \ref{fig:exp}). We measure a signal of $20\, \sigma$ in the decoded image. Thus:
\begin{equation}
\begin{array}{l}
S_{2\sigma}^{MC} (511\, keV) = 1.0 \times  10^{-4}\, ph\, cm^{-2}\, s^{-1} \\
Data: ISGRI \qquad rev.\, 50 \qquad exp. = 10\, Ms \\
Method: Monte\, Carlo\, simulation 
\end{array}
\end{equation}
Since we have used an estimation of the background taken during the first IBIS observations, this value is an estimation of the sensitivity in the early time of the INTEGRAL life, when the background was lower than now (Fig. \ref{fig:bkg}).

   The evaluation of the sensitivity that we have given using a Monte Carlo simulation is in substantial agreement with what is obtained using other methods, but the result can be made more accurate by adding to the real data the event file generated by the Monte Carlo code. Indeed, in making a more realistic simulation, we take into account the background dis-uniformity on the ISGRI detector plane  and we use the same  software both for data analysis and simulation. 

   A simulation of a 511~keV point source as should be observed during the 50th and 600th orbits of INTEGRAL satellite, is shown in figure \ref{fig:mc-and-data}. Using one millions 511~keV photons in the Monte Carlo, we detect in the early and late IBIS observations $10\, \sigma$ and $7\, \sigma$ 511~keV signals respectively. We could get with these simulation a flux estimation with an error of $\sim\, 10\, \%$. In order to have a better estimation we made another simulation with 10 million photons in the Monte Carlo input, reaching a flux error of $\sim\, 1\, \%$, which is fully appropriate for our purpose. With a source intensity corresponding to 10 million photons incident on an area equal to the surface of the mask ($11320\, cm^{2}$) we obtain a signal with a significance of $103\, \sigma$ during revolution 50. Taking into account the exposure ($1623\, s$) of the given observation, the short timescale sensitivity is equal to: 
\begin{equation}
\begin{array}{l}
S_{2\sigma}^{MC+data}  = 1.1 \times 10^{-2}\, ph\, cm^{-2}\, s^{-1} \\
Data: ISGRI \qquad rev.\, 50 \qquad exp. = 1623\, s \\
Method: Monte\, Carlo\, and\, data 
\end{array}
\label{eq:sens-scw}
\end{equation}
This number gives an indication on the flux that we need to have any evidence of a 511~keV signal with just one IBIS pointing, in a kilosecond timescale.

   Since the sensitivity goes as the square root of exposure (equation \ref{eq:sens}), we obtain for a $10\, Ms$ exposure the sensitivity: 
\begin{equation}
S_{2\sigma}^{MC+data} = 1.4 \times 10^{-4}\, ph\, cm^{-2}\, s^{-1} \;\; rev.\, 50 \; exp. = 10\, Ms
\end{equation}

   This measure refers to the first year of life INTEGRAL, when the background was less than in the more recent data (Fig. \ref{fig:bkg}). Simulating a measure of the same 511~keV flux  at the end of our data sets we get a $72\, \sigma$. Thus we estimate the sensitivity: 

\begin{equation}
S_{2\sigma}^{MC+data} = 2.0 \times 10^{-4}\, ph\, cm^{-2}\, s^{-1} \;\; rev.\, 600 \; exp. = 10\, Ms
\end{equation}

   The average value of these two numbers provides a more accurate estimate of sensitivity that we obtain with our data set: 
\begin{equation}
\begin{array}{l}
S_{2\sigma}^{MC+data} =  1.7 \times 10^{-4}\, ph\, cm^{-2}\, s^{-1}  \\
Data: ISGRI \qquad exposure = 10\, Ms \\
Method: Monte\, Carlo\, and\, data 
\end{array}
\end{equation}


==> table-example.tex <==
\begin{table*}
\caption{\label{t7}Spectral types and photometry for stars in the
  region.}
\centering
\begin{tabular}{lccc}
\hline\hline
Star&Spectral type&RA(J2000)&Dec(J2000)\\
\hline
69           &B1\,V     &09 15 54.046 & $-$50 00 26.67\\
49           &B0.7\,V   &*09 15 54.570& $-$50 00 03.90\\
LS~1267~(86) &O8\,V     &09 15 52.787&11.07\tablefootmark{a}\\
24.6         &7.58\tablefootmark{1}&1.37\tablefootmark{a}   &0.20\tablefootmark{a}\\
\hline
LS~1262      &B0\,V     &09 15 05.17&11.17\tablefootmark{b}\\
MO 2-119     &B0.5\,V   &09 15 33.7 &11.74\tablefootmark{c}\\
LS~1269      &O8.5\,V   &09 15 56.60&10.85\tablefootmark{d}\\
\hline
\end{tabular}
\tablefoot{ The top panel shows likely members of Pismis~11. The second
panel contains likely members of Alicante~5. The bottom panel
displays stars outside the clusters.\\
\tablefoottext{a}{Photometry for MF13, LS~1267 and HD~80077 from
Dupont et al.}
\tablefoottext{b}{Photometry for LS~1262, LS~1269 from
Durand et al.}
\tablefoottext{c}{Photometry for MO2-119 from
Mathieu et al.}
}
\end{table*}

==> table-mqs-delux.tex <==
\begin{deluxetable}{l r r c r r c c}
\tabletypesize{\footnotesize}
\tablecaption{511 keV $2\,\sigma$ steady flux upper limits for the hard X (E > 20~keV) microquasars reported in the 3rd IBIS catalogue}
\tablewidth{0pt}

\tablecolumns{7}

\tablehead{

\colhead{Source name}  & 
\colhead{R.A.} & 
\colhead{Dec} &
\colhead{Error\tablenotemark{a}} &
\colhead{$F_{20-40}$\tablenotemark{b}} &
\colhead{$F_{40-100}$} &
\colhead{$2\,\sigma$ flux limit\tablenotemark{c}} &
\colhead{Type\tablenotemark{d}} \\

\colhead{} & 
\colhead{(deg)} & 
\colhead{(deg)} &
\colhead{} &
\colhead{(mCrab)} &
\colhead{mCrab} & 
\colhead{($10^{-4}\,ph\,cm^{-2}\,s^{-1}$)} &
\colhead{} 

}\startdata
XTE J1550-564  & 237.745 & -56.479  & 0.2 & $34.0 \pm 0.1$  & $55.3 \pm 0.2$ & 2.7 & LMXB \\       

Sco X-1        & 244.980 & -15.643  & 0.2 & $685.7 \pm 0.3$ & $24.7 \pm 0.3$ & 3.7 & LMXB  \\        

GRO J1655-40   & 253.504 & -39.846  & 0.6 & $2.3 \pm 0.1$   & $2.7 \pm 0.2$  & 2.5 & LMXB  \\        

GX 339-4       & 255.706 & -48.792  & 0.3 & $40.7 \pm 0.1$  & $46.7 \pm 0.2$ & 2.6 & LMXB  \\       

1E 1740.7-2942 & 265.978 & -29.750 & 0.2 & $29.8 \pm 0.1$  & $36.6 \pm 0.1$ & 1.6 & LMXB  \\       

GRS 1758-258   & 270.303 & -25.746  & 0.3 & $58.8 \pm 0.1$  & $75.3 \pm 0.1$ & 1.6 & LMXB  \\         

SS 433         & 287.956 & 4.983    & 0.5 & $10.4 \pm 0.1$  & $5.2 \pm 0.2$  & 2.4 & HMXB  \\      

GRS 1915+105   & 288.799 & 10.944 & 0.2  & $296.8 \pm 0.1$ & $123.4 \pm 0.2$  & 2.5 & LMXB  \\      

Cyg X-1        & 299.590 & 35.199   & 0.2 & $763.7 \pm 0.2$ & $876.7 \pm 0.3$  & 3.0 & HMXB  \\       

Cyg X-3        & 308.108 & 40.956   & 0.2 & $196.5 \pm 0.2$ & $78.3 \pm 0.3$   & 2.6 & HMXB \\     
 \enddata

\tablenotetext{a}{Position error expressed as radius of 90 \% confidence circle in arcminutes}
\tablenotetext{b}{Fluxes averaged on the total exposure \citep{Bird2007}: \\ 
      20-40 keV: $1\,mCrab = 7.57 \times 10^{-12}\,erg\,cm^{-2}\,s^{-1} = 1.71 \times 10^{-4}\,ph\,cm^{-2}\,s^{-1}$ \\
      40-100 keV: $1\,mCrab = 9.42 \times 10^{-12}\,erg\,cm^{-2}\,s^{-1} = 9.67 \times 10^{-5}\,ph\,cm^{-2}\,s^{-1}$}
\tablenotetext{c}{The collective flux limit, obtained adding  the detected flux from all the sources, is $\; \sim\, 10^{-4}\,ph\,cm^{-2}\,s^{-1}$}
\tablenotetext{d}{Type identifiers: LMXB=Low Mass X-ray binary, HMXB=High Mass X-ray binary}
%\tablenotetext{b}{Type identifiers: LMXB=Low Mass X-ray binary, HMXB=High Mass X-ray binary, $\mu QSO$=Microquasars, T=transient, A=Atoll source, B=burster (neutron star), BHC=Black hole candidate, CV=Cataclysmic variable, D=Dipping source, G=Globular cluster X-ray source, PSR=Radio pulsar, PWN=Pulsar wind nebula,SGR=Soft Gamma Repeater, SNR = Supernova remnant, U=Ultrasoft source, XP=X-ray pulsar, Z=Z-type source (neutron stars).}
\label{tab:microquasars}
\end{deluxetable}


==> table-sgra-delux.tex <==
\begin{deluxetable}{l c c c c c}
\tabletypesize{\footnotesize}
\tablecaption{511 keV $2\,\sigma$ Sgr A* upper flux limit in the Galactic Center visibility periods.}
\tablewidth{0pt}

\tablecolumns{6}

\tablehead{

\colhead{Period}  & 
\colhead{Start Time} & 
\colhead{End Time} &
\colhead{No. ScWs\tablenotemark{a}} &
\colhead{Sgr A* Exposure\tablenotemark{b}} &
\colhead{Flux limit} \\

\colhead{} & 
\colhead{(UT)} & 
\colhead{(UT)} &
\colhead{} &
\colhead{(Ms)} &
\colhead{($10^{-4}\,ph\,cm^{-2}\,s^{-1}$)} 

}\startdata
 2003 Spring & 2003-02-28 & 2003-04-23 & 1731 & 0.650 & 5.7 \\
 2003 Autumn & 2003-08-10 & 2003-10-14 & 1717 & 1.872 & 3.2 \\
 2004 Spring & 2004-02-16 & 2004-04-20 & 1862 & 1.046 & 4.5 \\
 2004 Autumn & 2004-08-17 & 2004-10-27 & 2191 & 1.292 & 4.3 \\
 2005 Spring & 2005-02-16 & 2005-04-28 & 2144 & 1.165 & 4.7 \\
 2005 Autumn & 2005-08-16 & 2005-10-26 & 1667 & 0.790 & 5.9 \\
 2006 Spring & 2006-02-09 & 2006-04-25 & 1869 & 1.501 & 4.1 \\
 2006 Autumn & 2006-08-16 & 2006-11-02 & 1770 & 1.080 & 5.0 \\
 2007 Spring & 2007-02-01 & 2007-04-22 &  985 & 0.347 & 9.2 \\
 %2007 Autumn & 2007-08-19 & 2007-10-15 & ...& ...& ... \\
 \enddata
\tablenotetext{a}{Each ScW lasts about half an hour}
\tablenotetext{b}{Obtained from the exposure map. The exposure map, and in particular the value in the Galaxy depends both on the number of ScWs and the dithering patterns}
\label{tab:gcvis}
\end{deluxetable}


==> table-sn-delux.tex <==
\begin{deluxetable}{l r r c r r c}
\tabletypesize{\footnotesize}
\tablecaption{511 keV $2\,\sigma$ steady flux upper limits for the hard X (E > 20~keV) Supernova Remnants (SNR) reported in the 3rd IBIS catalogue.}
\tablewidth{0pt}

\tablecolumns{7}

\tablehead{

\colhead{Source name}  & 
\colhead{R.A.} & 
\colhead{Dec} &
\colhead{Error\tablenotemark{a}} &
\colhead{$F_{20-40}$\tablenotemark{b}} &
\colhead{$F_{40-100}$} &
\colhead{$2\,\sigma$ flux limit\tablenotemark{c}}  \\

\colhead{} & 
\colhead{(deg)} & 
\colhead{(deg)} &
\colhead{(arcminutes)} &
\colhead{(mCrab)} &
\colhead{mCrab} & 
\colhead{($10^{-4}\,ph\,cm^{-2}\,s^{-1}$)} 

}\startdata
4U 0022+63           &         6.319    &   64.159   &     3.6   &   $0.7 \pm 0.1$    &     $0.7 \pm 0.2$     &      2.3 \\
PSR J1811-1926    &    272.827     &  19.417    &    2.9    &  $0.8 \pm 0.1$     &    $1.0 \pm 0.2$      &    14  \\
IGR J18135-1751   &   273.395      & -17.871   &     2.2    &  $1.1 \pm 0.1$     &   $1.7 \pm 0.2$      &    2.3 \\
SNR 021.5-00.9      &   278.388      & -10.579   &     1.2    &  $3.3 \pm 0.1$     &    $3.3 \pm 0.2$     &     3.0 \\
AX J1838.0-0655  &   279.509     &   -6.916     &    1.5     &   $1.9 \pm 0.1$     &    $3.0 \pm 0.2$     &     2.9 \\
Kes 73                    &  280.338     & -4.948        &    1.3     &   $2.2 \pm 0.1$     &    $4.2 \pm 0.2$     &     2.9 \\
AX J1846.4-0258   &   281.596   &  -2.983       &      1.8    &  $1.7 \pm 0.1$     &    $2.4 \pm 0.2$      &    2.8 \\
Cas A                    &   350.848    & 58.815      &      0.9    &  $4.1 \pm 0.1$      &   $2.4 \pm 0.2$       &   2.5 
\enddata

\tablenotetext{a}{Position error expressed as radius of 90 \% confidence circle.}
\tablenotetext{b}{Fluxes averaged on the total exposure \citep{Bird2007}: \\ 
      20-40 keV: $1\,mCrab = 7.57 \times 10^{-12}\,erg\,cm^{-2}\,s^{-1} = 1.71 \times 10^{-4}\,ph\,cm^{-2}\,s^{-1}$ \\
      40-100 keV: $1\,mCrab = 9.42 \times 10^{-12}\,erg\,cm^{-2}\,s^{-1} = 9.67 \times 10^{-5}\,ph\,cm^{-2}\,s^{-1}$}
\tablenotetext{c}{The collective flux limit, obtained adding  the detected flux from all the sources, is $\; \sim\,10^{-4}\,ph\,cm^{-2}\,s^{-1}$}
\label{tab:snr}
\end{deluxetable}

